Attack-Resilient Weighted $\ell_1$ Observer with Prior Pruning

Security related questions for Cyber Physical Systems (CPS) have attracted much research attention in searching for novel methods for attack-resilient control and/or estimation. Specifically, false data injection attacks (FDIAs) have been shown to be capable of bypassing bad data detection (BDD), while arbitrarily compromising the integrity of state estimators and robust controller even with very sparse measurements corruption. Moreover, based on the inherent sparsity of pragmatic attack signals, $\ell_1$-minimization scheme has been used extensively to improve the design of attack-resilient estimators. For this, the theoretical maximum for the percentage of compromised nodes that can be accommodated has been shown to be $50\%$. In order to guarantee correct state recoveries for larger percentage of attacked nodes, researchers have begun to incorporate prior information into the underlying resilient observer design framework. For the most pragmatic cases, this prior information is often obtained through some data-driven machine learning process. Existing results have shown strong positive correlation between the tolerated attack percentages and the precision of the prior information. In this paper, we present a pruning method to improve the precision of the prior information, given corresponding stochastic uncertainty characteristics of the underlying machine learning model. Then a weighted $\ell_1$-minimization is proposed based on the pruned prior. The theoretical and simulation results show that the pruning method significantly improves the observer performance for much larger attack percentages, even when moderately accurate machine learning model used.

==> 2-Problem_Statement.tex <==
A physical attacked dynamic model of CPS can be given:
\begin{equation}\label{equ:system_model}
\begin{aligned}
    \mathbf{x}_{i+1} &= A\mathbf{x}_i \\
    \mathbf{y}_i &= C\mathbf{x}_i + \mathbf{e}_i
    \end{aligned}
\end{equation}
where, $\mathbf{x}_k \in \mathbb{R}^n, \mathbf{y}_k \in \mathbb{R}^m$, with $m >n$, denote state vector and measurement vector at time $i$ respectively, $\mathbf{e}_k \in \mathscr{S}_k^m$ denotes the sparse attack vector, $A,C$ are system dynamic parameters. A control input may be included in the model above. However, since the control input is generally irrelevant to state estimation problems, we suppress in the model considered here. By iterating the system model \eqref{equ:system_model} $T$ time steps, the $T$ horizon observation model is given 
\begin{equation}\label{equ:measurement_model}
    \mathbf{y}_T = H\mathbf{x}_{i-T+1}+\mathbf{e}_T
\end{equation}
where $\mathbf{y}_T=[\mathbf{y}_i^{\top} \hspace{2mm} \mathbf{y}_{i-1}^{\top} \cdots \mathbf{y}_{i-T+1}^{\top}]^{\top} \in \mathbb{R}^{Tm}$ is a sequence of observation in the moving window $[i-T+1 \hspace{2mm} i]$, $\mathbf{x}_{i-T+1}\in \mathbb{R}^n$ is the state vector at time $i-T+1$, $\mathbf{e}_T = [\mathbf{e}_i^{\top} \hspace{2mm} \mathbf{e}_{i-1}^{\top} \cdots \mathbf{e}_{i-T+1}^{\top}]^{\top} \in \mathscr{S}^{Tm}_{k}$ is the sequence of attack vectors in the same moving window with $\mathbf{e}_i \in \mathscr{S}_{k/T}^m, \forall i \in [i-T+1 \hspace{2mm} i]$ and
$$ H = \begin{bmatrix} C \\ C A \\ \vdots \\ C A^{T-1} \end{bmatrix} =U \begin{bmatrix} \Sigma_1 \\0\end{bmatrix}V^{\top}
$$
where, $U = [U_1 \hspace{2mm} U_2]$, with $U_1 \in {\mathbb R}^{Tm \times n}, U_2 \in {\mathbb R}^{Tm \times Tm-n}$, is a matrix of left singular vectors of $H$, $V \in \mathbb{R}^{n \times n}$ is the corresponding matrix of right singular vectors, $\Sigma_1 \in \mathbb{R}^{n \times n}$ is a diagonal matrix of the singular values of $H$, which are non-zero since $H$ is full rank.

\begin{definition}[Decoder]
Given a sequence of observation $\mathbf{y}_T \in \mathbb{R}^{Tm}$, the decoder for the measurement model in \eqref{equ:measurement_model} is a mapping of the form $\mathscr{D}:\mathbb{R}^{Tm} \mapsto \mathbb{R}^n$ given by
\begin{equation}\label{equ:decoder}
    \hat{\mathbf{x}} = \mathscr{D}(\mathbf{y}_T) =V\Sigma_1^{-1}\argmin_{\mathbf{z}}\|\mathbf{y}_T-U_1\mathbf{z}\|_{\ell_1}
\end{equation}
\end{definition}

\begin{definition}[Detector]
Given a positive threshold parameter $\epsilon$, a detector for the decoder $\mathscr{D}$ and the measurement model in \eqref{equ:measurement_model} is a binary classifier of the form
\begin{equation}\label{equ:detector}
    \mathscr{D}_{\epsilon}(\mathbf{y}_T) = \left\{
     \begin{array}{lr}
     1 &\quad\text{if}\hspace{0.2cm} \|\mathbf{y}_T - H\mathscr{D}(\mathbf{y}_T)\|_{\ell_1} > \epsilon \\
     0 &\quad\text{otherwise}
     \end{array}
     \right.
\end{equation}
\end{definition}

\begin{remark}
The positive class for $\mathscr{D}_{\epsilon}(\cdot)$ is the set of attacked (unsafe) measurements, while the negative class is the set of safe measurements.
\end{remark}

False data injection attack is modeled as an addictive bias through $\mathbf{e}$ on the sparse measurement nodes. We will assume the attacker has knowledge of system $(A,C)$. 

\begin{definition}[Successful FDIA \cite{mo2010false}]\label{Def:Successful_FDIA}
Consider the CPS in \eqref{equ:system_model} and the corresponding measurement model \eqref{equ:measurement_model}, the attack sequence $\mathbf{e}_T\in\mathscr{S}^{Tm}_{k}$ is said to be $(\epsilon, \alpha)$-successful against the decoder-detector pair $\{\mathscr{D}, \mathscr{D}_{\epsilon}\}$ if
\begin{equation}\label{equ:def_success_FDIA}
     \|\mathbf{x}^{\star}-\mathscr{D}(\mathbf{y}_T)\| \geq \alpha, \hspace{2mm} \mathscr{D}_{\epsilon}(\mathbf{y}_T)=0,
\end{equation}
where $\mathbf{y}_T = \mathbf{y}^{\star}_T+\mathbf{e}_T$ with $\mathbf{y}^*_T\in\mathbb{R}^{N}$ the true measurement vector, and $\mathbf{x}^{\star}$ is the true state vector.
\end{definition}

\begin{remark}
$(\epsilon,\alpha)$-successful FDIA can result in a state bias of size at least $\alpha$ while by-passing the detector $\mathscr{D}_{\epsilon}(\cdot)$.
\end{remark}

The following theorem gives a machanism for constructing such $(\epsilon,\alpha)$-successful FDIA if the attack support is pre-determined.

\begin{theorem}\label{Thm:FDIA}
Given the support sequence $\mathscr{T} = \{\mathscr{T}_i \hspace{2mm} \mathscr{T}_{i-1} \cdots \mathscr{T}_{i-T+1}\}$ with $|\mathscr{T}_i|\leq k$. Let $\mathbf{z}_e$ be an optimal solution of the optimization program
\begin{equation}\label{equ:FDIA_optimization}
\begin{aligned}
    \textsf{Maxmize}&: \hspace{0.2cm} \|\Sigma_1^{-1} \mathbf{z}\|_{\ell_2}, \\
    \textsf{Subject to}&: \hspace{0.2cm} \|U_{1,\mathscr{T}^c} \mathbf{z}\|_{\ell_2} \leq \epsilon.
\end{aligned}
\end{equation}
If $\bar{\sigma}_{\mathscr{T}^c}\sqrt{Tm-|\mathscr{T}|}<1$, then the FDIA
\begin{equation}\label{equ:FDIA}
    \mathbf{e}_{\mathscr{T}} = U_{1,\mathscr{T}} \cdot \mathbf{z}_e, \hspace{2mm} \mathbf{e}_{\mathscr{T}^c} = \mathbf{0}
\end{equation}
is $(\epsilon, \alpha)$-successful against the decoder-detector pair $\{\mathscr{D},\mathscr{D}_\epsilon\}$, with 
$$ \alpha = \frac{\epsilon}{\underline{\sigma}\overline{\sigma}_{\mathscr{T}^c}}(1-\overline{\sigma}_{\mathscr{T}^c}\sqrt{Tm-|\mathscr{T}|}),
$$
where $\overline{\sigma}_{\mathscr{T}^c}$ is the largest singular value of $U_{1,\mathscr{T}^c}$ and $\underline{\sigma}$ is the smallest nonzero singular value of $H$.
\end{theorem}
\begin{proof}
Since 
$$ \left\{\mathbf{z}\,\middle\vert\ \|\mathbf{z}\|_{\ell_2}\leq \frac{\epsilon}{\overline{\sigma}_{\mathscr{T}^c}}\right\} \subset \left\{\mathbf{z}\,\middle\vert\ \|U_{1,\mathscr{T}^c}\mathbf{z}\|_{\ell_2} \leq \epsilon\right\},
$$
where $\overline{\sigma}_{\mathscr{T}^c}$ is the largest singular value of $U_{1,\mathscr{T}^c}$, then
$$\|\Sigma_1^{-1} \mathbf{z}_e\|_{\ell_2} \geq \max_{\|\mathbf{z}\|_{\ell_2} \leq \frac{\epsilon}{\overline{\sigma}_{\mathscr{T}^c}}} \|\Sigma_1^{-1}\mathbf{z}\|_{\ell_2} \geq \frac{\epsilon}{\underline{\sigma}\overline{\sigma}_{\mathscr{T}^c}}
$$
Also
$$
    \hat{\mathbf{x}} = \mathscr{D}\left(\mathbf{y}^{\star}_T+P\begin{bmatrix}U_{1,\mathscr{T}} \\ 0\end{bmatrix}\mathbf{z}_e\right)
$$
for an appropriate permutation matrix $P$ satisfying $U_1 = P\begin{bmatrix}U_{1,\mathscr{T}} \\ U_{1,\mathscr{T}^c}\end{bmatrix}$. Hence
$$\begin{aligned}\hat{\mathbf{x}} &= V \Sigma_1^{-1} \argmin_{\mathbf{z}}\left\|U_1(\mathbf{z}^{\star}+\mathbf{z}_e+\mathbf{z}) - P\begin{bmatrix}0\\ U_{1,\mathscr{T}^c}\end{bmatrix}\mathbf{z}_e\right\|_{\ell_1} \\
&= V\Sigma_1^{-1}(\mathbf{z}^{\star}+\mathbf{z}_e-\mathbf{z}_e^{\perp})
\end{aligned}$$
where $\mathbf{z}^{\star}=\Sigma_1 V^{\top}\mathbf{x}^{\star}$ corresponds to the true state and $\mathbf{z}_e^{\perp}$ is the projection given by 
$$\mathbf{z}_e^{\perp} =\argmin_{\mathbf{z}}\left\|U_1\mathbf{z} - P\begin{bmatrix}0\\ U_{1,\mathscr{T}^c}\end{bmatrix}\mathbf{z}_e\right\|_{\ell_1}
$$
Thus,
$$\begin{aligned}\|\hat{\mathbf{x}}\|_{\ell_2} &= \|\Sigma_1^{-1}(\mathbf{z}_e-\mathbf{z}_e^{\perp})\|_{\ell_2} \\
&\geq \|\Sigma_1^{-1}\mathbf{z}_e\|_{\ell_2}-\|\Sigma_1^{-1}\mathbf{z}_e^{\perp}\|_{\ell_2} \geq \frac{\epsilon}{\underline{\sigma}\overline{\sigma}_{\mathscr{T}^c}} - \frac{1}{\underline{\sigma}}\|\mathbf{z}_e^{\perp}\|_{\ell_2}
\end{aligned}$$
Note\footnote{Let $f(\mathbf{z}) = \left\|U_1\mathbf{z} - P\begin{bmatrix}0\\ U_{1,\mathscr{T}^c}\end{bmatrix}\mathbf{z}_e\right\|_{\ell_1}$ which is a convex function.The unique minimizer $\mathbf{z}_e^{\perp}$ satisfies $f(\mathbf{z}_e^{\perp}) \le f(0)$.}
$$\begin{aligned} \|\mathbf{z}_e^{\perp}\|_{\ell_2} \leq \|\mathbf{z}_e^{\perp}\|_{\ell_1} &\leq \|U_{1,\mathscr{T}^c} \mathbf{z}_e\|_{\ell_1} \\
&\leq \sqrt{Tm-|\mathscr{T}|} \cdot \|U_{1,\mathscr{T}^c} \mathbf{z}_e\|_{\ell_2} \\
&\leq (\sqrt{Tm-|\mathscr{T}|}) \epsilon
\end{aligned}$$
Therefore,
$$\begin{aligned}\|\hat{\mathbf{x}}-\mathbf{x}^{\star}\|_{\ell_2} &\geq \frac{\epsilon}{\underline{\sigma}\overline{\sigma}_{\mathscr{T}^c}}-\frac{\epsilon}{\underline{\sigma}}\sqrt{Tm-|\mathscr{T}|} \\
 &\geq \frac{\epsilon}{\underline{\sigma}}\left(\frac{1}{\overline{\sigma}_{\mathscr{T}^c}}-\sqrt{Tm-|\mathscr{T}|}\right) \triangleq \alpha
\end{aligned}$$
Moreover,
$$\begin{aligned}
\|\mathbf{y}_T &-H\hat{\mathbf{x}}\|_{\ell_1} =\left\|U_1(\mathbf{z}^{\star}+\mathbf{z}_e)-P\begin{bmatrix}0\\ U_{1,\mathscr{T}^c}\end{bmatrix}\mathbf{z}_e-H\hat{\mathbf{x}}\right\|_{\ell_1} \\
&=\left\|U_1(\mathbf{z}^{\star}+\mathbf{z}_e)-P\begin{bmatrix}0\\ U_{1,\mathscr{T}^c}\end{bmatrix}\mathbf{z}_e-U_1(\mathbf{z}^{\star}+\mathbf{z}_e-\mathbf{z}_e^{\perp})\right\|_{\ell_1}\\
& = \left\|U_1\mathbf{z}_e^{\perp}-P\begin{bmatrix}0\\ U_{1,\mathscr{T}^c}\end{bmatrix}\mathbf{z}_e\right\|_{\ell_1} \leq \sqrt{Tm-|\mathscr{T}|} \cdot \overline{\sigma}_{\mathscr{T}^c}\epsilon
\end{aligned}$$
So, if $\bar{\sigma}_{\mathscr{T}^c}\sqrt{Tm-|\mathscr{T}|}<1$, then $\|\mathbf{y}_T -H\hat{\mathbf{x}}\|_{\ell_1} \leq \epsilon$
\end{proof}



==> 3-Main_Result.tex <==
As discussed in \emph{Section \ref{Sec: Introduction}}, we start from modeling the uncertainty of machine learning localization result (\emph{Support Prior}), then a pruning method is given to generate a new estimated support (\emph{Prune Support Prior}), with precision improvement. Finally, a weighted $\ell_1$ observer is given based on \emph{Prune Support Prior}.

Assume the actual support of safe nodes is represented by $\mathscr{T}^c$, let the vector $\mathbf{q}\in\{0,1\}^{Tm}$ be an indicator of the support $\mathscr{T}$, such that
 \begin{equation} \label{equ:support_indicator}
     \mathbf{q}_{i}=\left\{
     \begin{array}{lr}
     1 &\quad\text{if}\hspace{0.2cm} i \in \mathscr{T}^{c} \\
     0 &\quad\text{otherwise}
     \end{array}
     \right.
 \end{equation}
 
 The outputted \emph{Support Prior} $\hat{\mathscr{T}}^c$ of any underlying machine learning localization algorithm is an estimate of $\mathscr{T}^c$, and the estimated indicator $\hat{\mathbf{q}}\in\{0,1\}^{Tm}$ is defined similarly to \eqref{equ:support_indicator}. Then an uncertainty model is defined as
  \begin{equation} \label{equ:uncertainty_model}
     \mathbf{q}_{i}=\epsilon_{i}\hat{\mathbf{q}}_{i}+(1-\epsilon_{i})(1-\hat{\mathbf{q}}_{i})
 \end{equation}
 where $\epsilon_i \sim \mathscr{B}(1,\mathbf{p}_i)$, with known $\mathbf{p}_i \in {\mathbb R}_{+}$, and $E[\mathbf{p}_i] = T_r$, where $T_r$ is \emph{true rate} obtained from the \emph{Receiver Operator Characteristic} (ROC) of the underlying machine learning algorithm.
\begin{definition}[Positive Prediction Value, Precision, $\textsf{PPV}$]\label{Def:PPV_def}
Given an prior support knowledge $\hat{\mathbf{q}}\in\{0,1\}^N$ of an unknown attack support indicator $\mathbf{q}\in\{0,1\}^N$, $\textsf{PPV}$ is the proportion of $\mathbf{q}$ that is correctly identified in $\hat{\mathbf{q}}$. It is given by
\begin{equation}\label{equ:PPV_def}
\textsf{PPV} =  \frac{\|\mathbf{q} \circ \hat{\mathbf{q}} \|_{\ell_0}}{\|\hat{\mathbf{q}}\|_{\ell_0}} 
\end{equation}
\end{definition}

\begin{lemma}(\cite{Zheng2020resilient})  \label{Lem:PBD_CDF}
Given mutually independent Bernoulli random variables $\epsilon_i \sim \mathscr{B}(1,\mathbf{p}_i)$, $i=1,\cdots,Tm$, then
  \begin{equation}\label{equ:PMF}
      \textsf{Pr}\left\{\sum_{i=1}^{Tm} \epsilon_{i} = k-1 \right\}=\mathbf{r}(k), k=1,\cdots,Tm+1
  \end{equation}
  where,
  $$ \mathbf{r} = \beta \cdot \begin{bmatrix}-\mathbf{s}_1\\1 \end{bmatrix} * \begin{bmatrix}-\mathbf{s}_2\\1 \end{bmatrix} * \cdots * \begin{bmatrix}-\mathbf{s}_{Tm}\\1 \end{bmatrix}
  $$
  with
  $ \beta =\displaystyle\prod_{i=1}^{Tm} \mathbf{p}_{i}, \hspace{2mm} \mathbf{s}_i = -\frac{1-\mathbf{p}_{i}}{\mathbf{p}_{i}}
  $
\end{lemma}

Next, based on the knowledge of uncertainty of \emph{Prior}, the pruning process will perform in two steps.
Firstly, given a reliability level $\eta \in (0,1)$, the maximum integer $l_{\eta} (\leq Tm)$ of safe nodes being correctly localized with a probability of at least $\eta$ is obtained:
\begin{equation}\label{equ:trust_number}
\begin{aligned}
    l_{\eta} &= \textsf{max} \left\{k \mid \textsf{Pr} \left\{\sum_{i\in \hat{\mathscr{T}}^c} \epsilon_{i} \geq k \right\}\geq \eta \right\} \\
    &= \textsf{max} \left\{k \mid \sum_{i=1}^{k+1} \mathbf{r}_{\hat{\mathscr{T}}^c}(i) \leq 1-\eta \right\}
\end{aligned}
\end{equation}
where $\mathbf{r}_{\hat{\mathscr{T}}^c}$ is given by \eqref{equ:PMF}, using the index set $\hat{\mathscr{T}}^c$.

Then a \emph{Prune Support Prior} is obtained through a robust extraction:
\begin{equation}    \label{equ:pruning_alg}
    \hat{\mathscr{T}}^{c}_{\eta} =  \big\{\textsf{argsort} \downarrow (\mathbf{p} \circ \hat{\mathbf{q}})\big\}_{1}^{l_{\eta}}
\end{equation}
where, $\{\cdot\}_{1}^{l_{\eta}}$ is an index extraction from the first elements to $l_{\eta}$ elements.

\begin{definition}[Weighted $\ell_1$ Observer with Pruned Prior]
Consider the CPS in \eqref{equ:system_model} and the corresponding measurement model \eqref{equ:measurement_model}, given \emph{Prune Support Prior} $\hat{\mathscr{T}}^{c}_{\eta}$ by \eqref{equ:pruning_alg}, a weighted $\ell_1$ observer is defined
\begin{equation}\label{equ:weighted_l1_minimization}
\begin{aligned}
\textsf{Minimize}_{\mathbf{z}\in \mathbb{R}^n}\hspace{1mm} \|\mathbf{y}_T - H \mathbf{z}\|_{\ell_1, \mathrm{w}}, \hspace{1mm} \text { with }  \mathrm{w}_{i}=\left\{\begin{array}{ll}
1, & i \in \hat{\mathscr{T}}^{c}_{\eta} \\
\omega, & i \in \hat{\mathscr{T}}_{\eta}
\end{array}\right.
\end{aligned}    
\end{equation}
where, $0\leq \omega \leq 1$, $\|\mathbf{z}\|_{1, \mathrm{w}} \triangleq \sum_i \mathrm{w}_i |\mathbf{z}_i|$ is the weighted $\ell_1$ norm. 
\end{definition}


\begin{theorem}\label{Thm:recovery_Withpruning}
Consider the system model in \eqref{equ:system_model} together with the corresponding measurement model \eqref{equ:measurement_model}. Assume there exists a \emph{Support Prior} $\hat{\mathscr{T}}^c$ generated by an underlying machine learning localization algorithm with uncertainty model in \eqref{equ:uncertainty_model} and
\begin{equation}\label{equ:conditon_ML}
    \sum_{i=1}^{Tm} \mathbf{p}_i > Tm \cdot p_A.
\end{equation}
Given a positive parameter $\eta$ satisfying
\begin{equation}    \label{equ:strict_condition_for_eta}
    \eta \leq 1-e \left(1-\frac{(e-1)\sum_{i\in \hat{\mathscr{T}}^c}\mathbf{p}_i}{e|\mathscr{T}^c|}\right)^{|\mathscr{T}^c|},
\end{equation}
where $e$ is Euler's number, a \emph{Pruned Support Prior} $\hat{\mathscr{T}}_{\eta}^c$ given by \eqref{equ:trust_number} and \eqref{equ:pruning_alg}. If there exists an integer $a\geq \max\left\{\rho-1,1\right\}$, where $\rho = \frac{|\hat{\mathscr{T}}_{\eta}|}{k}$, such that any coding matrix $F$ ($FH=0$) satisfies RIP condition
\begin{align}\label{equ: RIP}
   (1-\delta_{S})\|\mathbf{h}\|_{\ell_2}^2 \leq \|F_\mathscr{T}\mathbf{h}\|_{\ell_2}^2 \leq (1+\delta_{S})\|\mathbf{h}\|_{\ell_2}^2 
 \end{align}
for all sparse vector $\mathbf{h} \in \mathscr{S}^{Tm}_{S}$, and RIP constant satisfies
\begin{equation}
    \delta_{ak}-C\delta_{(a+1)k} \leq C-1
\end{equation} 
then, with a probability of at least $\eta$, the estimation error of the Weighted $\ell_1$ Observer in \eqref{equ:weighted_l1_minimization} can be upper bounded as
\begin{equation} \label{equ:error_bound3}
    \left\|\hat{\mathbf{x}}-\mathbf{x}\right\|_{\ell_2} \leq 
   \frac{C_{1}}{\underline{\sigma}_H\sqrt{k}}\left(\omega\sigma_k(\mathbf{e})_{\ell_1}+(1-\omega)\|\mathbf{e}_{\hat{\mathscr{T}}_{\eta}^c} \|_{\ell_1}\right),
\end{equation}
where $\underline{\sigma}_H$ is the smallest singular value of $H$, and 
$$\begin{aligned} C_1 &= \frac{2a^{-\frac{1}{2}}(\sqrt{1-\delta_{(a+1)k}}+\sqrt{1+\delta_{a k}})}{\sqrt{1-\delta_{(a+1)k}}-\frac{1}{C}\sqrt{1+\delta_{a k}}}, \\  C &= \frac{a}{(\omega+(1-\omega)\sqrt{\rho -1})^2}.
\end{aligned}$$
\end{theorem}

\begin{proof}
Expanding \eqref{equ:uncertainty_model} yields 
$$
\mathbf{q}_i = 2\epsilon_i \hat{\mathbf{q}}_i +1 -\hat{\mathbf{q}}_i-\epsilon_i
=2\mathbf{q}_i \hat{\mathbf{q}}_i+1-\hat{\mathbf{q}}_i-\epsilon_i
$$
This implies that
$$ \epsilon_i -1 +\mathbf{q}_i = 2(\mathbf{q}_i \hat{\mathbf{q}}_i-\frac{1}{2}\hat{\mathbf{q}}_i)
$$
Summing over $i=1,\cdots,Tm$ and taking expectation of both sides yield
$$ \sum_{i=1}^{Tm} \mathbf{p}_i -Tm +E[\|\mathbf{q}\|_{\ell_0}] = 2 E\left[\|\mathbf{q} \circ \hat{\mathbf{q}} \|_{\ell_0}-\frac{1}{2}\|\hat{\mathbf{q}}\|_{\ell_0}\right].
$$
Using the condition in \eqref{equ:conditon_ML} yields
$$ E\left[\|\mathbf{q} \circ \hat{\mathbf{q}} \|_{\ell_0}-\frac{1}{2}\|\hat{\mathbf{q}}\|_{\ell_0}\right] > 0
$$
which means $\textsf{PPV} > 1/2$, then 
$$\textsf{Pr}\{\mathbf{q}\circ \hat{\mathbf{q}}=1 \mid \hat{\mathbf{q}}=1\} >\textsf{Pr}\{\mathbf{q}\circ \hat{\mathbf{q}}=0 \mid \hat{\mathbf{q}}=1\}$$
and with the operation in \eqref{equ:pruning_alg}, it follows
$$ \hat{\mathscr{T}}^{c}_{\eta} \subseteq \hat{\mathscr{T}}^{c} \cap \mathscr{T}^c, \hspace{2mm} \text{if} \hspace{2mm} 0<l_{\eta}\leq \|\mathbf{q}\circ \hat{\mathbf{q}}\|
$$
From \eqref{equ:trust_number}, it is true that
\begin{equation}\label{equ1}
    \textsf{Pr}\{0 \leq l_{\eta}\leq \|\mathbf{q}\circ \hat{\mathbf{q}}\|\} \geq \eta,
\end{equation}
As well known, Poisson-binomial distribution can be approximated by Binomial distribution, such that
$$\sum_{i\in \hat{\mathscr{T}}^c} \epsilon_{i} \sim \mathscr{B}\left(|\mathscr{T}^c|,\frac{\sum_{i\in \hat{\mathscr{T}}^c} \mathbf{p}_i}{|\mathscr{T}^c|}\right)
$$
then, from condition \eqref{equ:strict_condition_for_eta}, $ \eta \leq 1-e\mathscr{M}_{\sum_{i\in \hat{\mathscr{T}}^c} \epsilon_{i}}(-1)$, where $\mathscr{M}_{\sum_{i\in \hat{\mathscr{T}}^c} \epsilon_{i}}(t)$ is the moment generating function of $\sum_{i\in \hat{\mathscr{T}}^c} \epsilon_{i}$, thus
$$ E\left[\exp{\left(1-\sum_{i\in \hat{\mathscr{T}}^c} \epsilon_{i}\right)}\right] \leq 1-\eta
$$
Since $\exp(z)\geq 1$ for any $z\geq 0$, we obtain $E[\exp(z)] \geq \textsf{Pr}(z\geq 0)$, then it yields
$$ \textsf{Pr} \left\{1-\sum_{i\in \hat{\mathscr{T}}^c} \epsilon_{i} \geq 0 \right\} \leq 1-\eta \hspace{1mm}\Leftrightarrow \hspace{1mm} \textsf{Pr} \left\{\sum_{i\in \hat{\mathscr{T}}^c} \epsilon_{i} \geq 1\right\} \geq \eta
$$
which means $l_{\eta} \neq 0$, combining with \eqref{equ1}, we obtain $\textsf{Pr}\{0 < l_{\eta}\leq \|\mathbf{q}\circ \hat{\mathbf{q}}\|\} \geq \eta$, thus, $\textsf{Pr}\{ \hat{\mathscr{T}}^{c}_{\eta} \subseteq \hat{\mathscr{T}}^{c} \cap \mathscr{T}^c \subseteq \mathscr{T}^c\} \geq \eta $, then
 \begin{equation}\label{equ:pruning_preceison_100}
     \textsf{Pr}\left\{\textsf{PPV}_{\eta} =1 \right\} \geq \eta
 \end{equation} 
 
To avoid repetition, we state upfront that all claims made in this rest of proof holds with a probability of at least $\eta$. Under this probability, we have $\hat{\mathscr{T}}^{c}_{\eta} \subset \mathscr{T}^c$, $\mathscr{T}\subset \hat{\mathscr{T}}_{\eta}$.

Let $\hat{\mathbf{x}}$ be a minimizer to \eqref{equ:weighted_l1_minimization} with $H\hat{\mathbf{x}} = H\mathbf{x}+\mathbf{h}$, then the corresponding attack vector $\mathbf{e}^{\star} = \mathbf{e}+\mathbf{h}$, thus $\|\mathbf{e}^{\star}\|_{\ell_1,\omega} \leq \|\mathbf{e}\|_{\ell_1,\omega}$. Following the definition of weight $w$ in \eqref{equ:weighted_l1_minimization}, 
$$\omega \|\mathbf{e}_{\hat{\mathscr{T}}_{\eta}}+\mathbf{h}_{\hat{\mathscr{T}}_{\eta}} \|_{\ell_1} + \|\mathbf{e}_{\hat{\mathscr{T}}^{c}_{\eta}}+\mathbf{h}_{\hat{\mathscr{T}}^{c}_{\eta}}\|_{\ell_1} \leq \omega \|\mathbf{e}_{\hat{\mathscr{T}}_{\eta}}\|_{\ell_1}
+ \|\mathbf{e}_{\hat{\mathscr{T}}^c_{\eta}}\|_{\ell_1}
$$
Since $\ell_1$ norm is decomposable for disjoint sets, such for $\mathscr{T}$ and $\mathscr{T}^c$, and $\hat{\mathscr{T}}^{c}_{\eta} \cap\mathscr{T} =\emptyset $, $\hat{\mathscr{T}}^{c}_{\eta} \cap \mathscr{T}^c =\hat{\mathscr{T}}^{c}_{\eta}$, $\mathscr{T}\cap \hat{\mathscr{T}}_{\eta}=\mathscr{T}$, it follows
$$\begin{aligned} \omega \|\mathbf{e}_{\mathscr{T}}+\mathbf{h}_{\mathscr{T}}\|_{\ell_1} +\omega\|\mathbf{e}_{\hat{\mathscr{T}}_{\eta} \cap \mathscr{T}^c}+\mathbf{h}_{\hat{\mathscr{T}}_{\eta} \cap \mathscr{T}^c}\|_{\ell_1} + \|\mathbf{e}_{\hat{\mathscr{T}}^{c}_{\eta}}+\mathbf{h}_{\hat{\mathscr{T}}^{c}_{\eta}}\|_{\ell_1} \\
\leq \omega\|\mathbf{e}_{\mathscr{T}}\|_{\ell_1} +\omega \|\mathbf{e}_{\hat{\mathscr{T}}_{\eta}\cap \mathscr{T}^c}\|_{\ell_1} +\|\mathbf{e}_{\hat{\mathscr{T}}^c_{\eta}}\|_{\ell_1}
\end{aligned}$$
By triangle inequality, it follows
$$ \omega\|\mathbf{h}_{\hat{\mathscr{T}}_{\eta} \cap \mathscr{T}^c}\|_{\ell_1}+\|\mathbf{h}_{\hat{\mathscr{T}}_{\eta}^c}\|_{\ell_1} \leq \omega \|\mathbf{h}_{\mathscr{T}}\|_{\ell_1} +2\left(\|\mathbf{e}_{\hat{\mathscr{T}}_{\eta}^c}\|_{\ell_1}+\omega\|\mathbf{e}_{\hat{\mathscr{T}}_{\eta} \cap \mathscr{T}^c}\|_{\ell_1}\right)
$$
Adding and subtracting $\omega\|\mathbf{h}_{\hat{\mathscr{T}}_{\eta}^c \cap \mathscr{T}^c}\|_{\ell_1} (= \omega\|\mathbf{h}_{\hat{\mathscr{T}}_{\eta}^c}\|_{\ell_1})$ on LHS, $2\omega\|\mathbf{e}_{\hat{\mathscr{T}}_{\eta}^c \cap \mathscr{T}^c}\|_{\ell_1} (= 2\omega\|\mathbf{e}_{\hat{\mathscr{T}}_{\eta}^c}\|_{\ell_1})$ on RHS, it yields
$$\begin{aligned}\omega\|\mathbf{h}_{\mathscr{T}^c}\|_{\ell_1}+(1-\omega)\|\mathbf{h}_{\hat{\mathscr{T}}_{\eta}^c}\|_{\ell_1} \leq  \omega\|\mathbf{h}_{\mathscr{T}}\|_{\ell_1} + \\ 2\left(\omega\|\mathbf{e}_{\mathscr{T}^c}\|_{\ell_1}+(1-\omega)\|\mathbf{e}_{\hat{\mathscr{T}}_{\eta}^c}\|_{\ell_1}\right)
\end{aligned}$$
And since $\|\mathbf{h}_{\mathscr{T}^c}\|_{\ell_1} = \omega\|\mathbf{h}_{\mathscr{T}^c}\|_{\ell_1}+(1-\omega)\|\mathbf{h}_{\hat{\mathscr{T}}_{\eta}^c}\|_{\ell_1}+ (1-\omega)\|\mathbf{h}_{\hat{\mathscr{T}}_{\eta} \cap \mathscr{T}^c}\|_{\ell_1}$, it yields
\begin{equation}\label{equ2}
    \begin{aligned} \|\mathbf{h}_{\mathscr{T}^c}\|_{\ell_1} \leq \omega\|\mathbf{h}_{\mathscr{T}}\|_{\ell_1} + (1-\omega)\|\mathbf{h}_{\hat{\mathscr{T}}_{\eta} \cap \mathscr{T}^c}\|_{\ell_1}+ \\ 2\left(\omega\|\mathbf{e}_{\mathscr{T}^c}\|_{\ell_1}+(1-\omega)\|\mathbf{e}_{\hat{\mathscr{T}}_{\eta}^c}\|_{\ell_1}\right)
\end{aligned}
\end{equation}
Next, sort the coefficients of $\mathbf{h}_{\mathscr{T}^c}$ in descending order, and let $\mathscr{T}_j, j\in \{1,2,\cdots\}$ denote $j$th support in $\mathbf{h}_{\mathscr{T}^c}$ with size $ak \in \mathbb{Z}$, where $a>1$. Since $\|\mathbf{h}_{\mathscr{T}_{j-1}}\|_{\ell_1} \geq ak \cdot \min_{i \in \mathscr{T}_{j-1}}(\mathbf{h}_{\mathscr{T}_{j-1}})_i \geq ak \|\mathbf{h}_{\mathscr{T}_{j}}\|_{\ell_{\infty}}$, let $\mathscr{T}_0 = \mathscr{T} \cup \mathscr{T}_1$, we have
\begin{equation}\label{equ3}
    \|\mathbf{h}_{\mathscr{T}_0^c}\|_{\ell_2} \leq \sum_{j\geq 2}\|\mathbf{h}_{\mathscr{T}_j}\|_{\ell_{\infty}} \leq ak^{-1/2}\sum_{j\geq 1}\|\mathbf{h}_{\mathscr{T}_j}\|_{\ell_{1}} =  ak^{-1/2}\|\mathbf{h}_{\mathscr{T}^c}\|_{\ell_{1}}
\end{equation} 
Note that $|\hat{\mathscr{T}}_{\eta} \cap \mathscr{T}^c|=(\rho-1)k $ since $\textsf{PPV}=1$, and $|\mathscr{T}| =k$, then $\|\mathbf{h}_{\hat{\mathscr{T}}_{\eta} \cap \mathscr{T}^c}\|_{\ell_1} \leq \sqrt{(\rho-1)k}\|\mathbf{h}_{\hat{\mathscr{T}}_{\eta} \cap \mathscr{T}^c}\|_{\ell_2}$ , $\|\mathbf{h}_{\mathscr{T}}\|_{\ell_1} \leq \sqrt{k}\|\mathbf{h}_{\mathscr{T}}\|_{\ell_2} \leq \sqrt{k}\|\mathbf{h}_{\mathscr{T}_0}\|_{\ell_2}$. Since $a \geq \rho-1$, we obtain $|\hat{\mathscr{T}}_{\eta} \cap \mathscr{T}^c|=(\rho-1)k \leq ak =|\mathscr{T}_1|$, 
then $\|\mathbf{h}_{\hat{\mathscr{T}}_{\eta} \cap \mathscr{T}^c}\|_{\ell_2} = \|\mathbf{h}_{\mathscr{T} \cup (\hat{\mathscr{T}}_{\eta} \cap \mathscr{T}^c)}\|_{\ell_2} \leq \|\mathbf{h}_{\mathscr{T}_0}\|_{\ell_2}$.
Then combine with \eqref{equ2} and \eqref{equ3},
\begin{equation}\label{equ4}
\begin{aligned}
    \|\mathbf{h}_{\mathscr{T}_0^c}\|_{\ell_2} \leq & \frac{\omega+(1-\omega)\sqrt{\rho-1}}{\sqrt{a}}\|\mathbf{h}_{\mathscr{T}_0}\|_{\ell_2} \\&+\frac{2}{\sqrt{ak}}\left(\omega\|\mathbf{e}_{\mathscr{T}^c}\|_{\ell_1}+(1-\omega)\|\mathbf{e}_{\hat{\mathscr{T}}_{\eta}^c}\|_{\ell_1}\right)
\end{aligned}\end{equation}


Since $ \|F\mathbf{h}\|_{\ell_2}=\|(F\mathbf{e}^{\star}-F\mathbf{y}_T)-(F\mathbf{e}-F\mathbf{y}_T)\|_{\ell_2} =0$, it follows, based on triangle inequality and RIP condition,
$$\begin{aligned} \sqrt{1-\delta_{(a+1)k}}\|\mathbf{h}_{\mathscr{T}_0}\|_{\ell_2} \leq \|F\mathbf{h}_{\mathscr{T}_0}\|_{\ell_2} \leq \|F\mathbf{h}_{\mathscr{T}_0^c}\|_{\ell_2} \leq \\
\sum_{j\geq 2} \|F\mathbf{h}_{\mathscr{T}_j}\|_{\ell_2} 
\leq \sqrt{1+\delta_{ak}}\sum_{j\geq 2} \|\mathbf{h}_{\mathscr{T}_j}\|_{\ell_2} \leq \frac{\sqrt{1+\delta_{ak}}}{\sqrt{ak}} \|\mathbf{h}_{\mathscr{T}^c}\|_{\ell_{1}}
\end{aligned}$$
Combining with \eqref{equ2}, it yields
$$\begin{aligned} \sqrt{1-\delta_{(a+1)k}}\|\mathbf{h}_{\mathscr{T}_0}\|_{\ell_2} \leq  \omega\frac{\sqrt{1+\delta_{ak}}}{\sqrt{ak}} \|\mathbf{h}_{\mathscr{T}}\|_{\ell_1} + \\ (1-\omega)\frac{\sqrt{1+\delta_{ak}}}{\sqrt{ak}} \|\mathbf{h}_{\hat{\mathscr{T}}_{\eta} \cap \mathscr{T}^c}\|_{\ell_1}\\ +2\frac{\sqrt{1+\delta_{ak}}}{\sqrt{ak}} \left(\omega\|\mathbf{e}_{\mathscr{T}^c}\|_{\ell_1}+(1-\omega)\|\mathbf{e}_{\hat{\mathscr{T}}_{\eta}^c}\|_{\ell_1}\right)
\end{aligned}
$$
Notice, we have $\|\mathbf{h}_{\mathscr{T}}\|_{\ell_1}\leq \sqrt{k}\|\mathbf{h}_{\mathscr{T}_0}\|_{\ell_2} $ and $\|\mathbf{h}_{\hat{\mathscr{T}}_{\eta} \cap \mathscr{T}^c}\|_{\ell_1} \leq \sqrt{(\rho-1)k}\|\mathbf{h}_{\mathscr{T}_0}\|_{\ell_2}$. Combining with the upper inequality,
$$ \|\mathbf{h}_{\mathscr{T}_0}\|_{\ell_2} \leq \frac{2\frac{\sqrt{1+\delta_{ak}}}{\sqrt{ak}} \left(\omega\|\mathbf{e}_{\mathscr{T}^c}\|_{\ell_1}+(1-\omega)\|\mathbf{e}_{\hat{\mathscr{T}}_{\eta}^c}\|_{\ell_1}\right)}{\sqrt{1-\delta_{(a+1)k}}-\frac{\omega+(1-\omega)\sqrt{\rho-1}}{\sqrt{a}}\sqrt{1+\delta_{ak}}}
$$
Since $\|\mathbf{h}\|_{\ell_2}\leq \|\mathbf{h}_{\mathscr{T}_0}\|_{\ell_2} +\|\mathbf{h}_{\mathscr{T}_0^c}\|_{\ell_2} $, combine the above inequality with \eqref{equ4}, it yields
$$ \|\mathbf{h}\|_{\ell_2}\leq \frac{2\frac{\sqrt{1-\delta_{(a+1)k}}+\sqrt{1+\delta+{ak}}}{\sqrt{ak}}\left(\omega\|\mathbf{e}_{\mathscr{T}^c}\|_{\ell_1}+(1-\omega)\|\mathbf{e}_{\hat{\mathscr{T}}_{\eta}^c}\|_{\ell_1}\right)}{\sqrt{1-\delta_{(a+1)k}}-\frac{\omega+(1-\omega)\sqrt{\rho-1}}{\sqrt{a}}\sqrt{1+\delta_{ak}}}
$$
where $\|\mathbf{e}_{\mathscr{T}^c}\|_{\ell_1} = \sigma_k(\mathbf{e})_{\ell_1}$ is best $k$ sparse approximation error of $\mathbf{e}$ defined in \eqref{equ:best_k_sparse_estimation_error}, and the estimation error $\|\hat{\mathbf{x}}-\mathbf{x}\|_{\ell_2} \leq \underline{\sigma}_H^{-1}\|\mathbf{h}\|_{\ell_2}$, and $\underline{\sigma}_H$ is the smallest singular value of $H$. Moreover, to maintain the denominator to be positive, a condition is given
$$ \delta_{ak} + C\delta_{(a+1)k} < C-1
$$
where $C = \frac{a}{(\omega+(1-\omega)\sqrt{\rho-1})^2}$.
\end{proof}
\begin{remark}
 The condition in \eqref{equ:conditon_ML} guarantees the underlying machine learning algorithm works better than random flip of a fair coin, which is a reasonable assumption.
\end{remark}

\begin{remark}
 A precision improvement conclusion \eqref{equ:pruning_preceison_100} is given in proof, and notice that the upper bound restriction of $\eta$ is an overwhelming probability.
\end{remark}

\begin{remark}
 To avoid the sacrifice of redundancy of measurements, we set weight $\omega$ close to zero, but not zero, even if we are confident in the precision of $\hat{\mathscr{T}}_{\eta}^c$.
\end{remark}

 
 
